$L_2$-small ball asymptotics for a family of finite-dimensional perturbations of Gaussian functions

In this article we study the small ball probabilities in $L_2$-norm for a family of finite-dimensional perturbations of Gaussian functions. We define three types of perturbations: non-critical, partially critical and critical; and derive small ball asymptotics for the perturbated process in terms of the small ball asymptotics for the original process. The natural examples of such perturbations appear in statistics in the study of empirical processes with estimated parameters (the so-called Durbin's processes). We show that the Durbin's processes are critical perturbations of the Brownian bridge. Under some additional assumptions, general results can be simplified. As an example we find the exact $L_2$-small ball asymptotics for critical perturbations of the Green processes (the processes which covariance function is the Green function of the ordinary differential operator).

==> S5-Gaussian.tex <==
\newpage
\section{Малые уклонения случайных гауссовских процессов}
%\addcontentsline{toc}{section}{Малые уклонения случайных гауссовских процессов}
\label{appendix:SBA}
Напомним основные определения и теоремы из теории $L_2$-малых уклонений для гауссовских случайных функций.

Пусть $X(x)$, $x\in \bar{\mathcal{O}}\subset \mathbb{R}^d$, --- гауссовская случайная функция с нулевым средним и функцией ковариации $G(x,y)=\mathbb{E}X(x)X(y)$. Предположим
\begin{align}
	\|X\|^2=\int\limits_{\mathcal{O}}X^2(x)\,dx<\infty\quad \text{п.н.}
\end{align}
Тогда для функции $X(x)$ справедливо разложение Кархунена--Лоэва\footnote{В литературе также встречается перевод <<разложение Карунена--Лоэва>>} (Karhunen--Lo{\`e}ve, см. напр.~\cite[\S 12]{lifshitz2016}), а именно, верно равенство п.н.:
\begin{align*}
	X(x)=\sum\limits_{k=1}^{\infty}\sqrt{\mu_k}u_k(x)\xi_k,\qquad x\in \mathcal{O},
\end{align*}
где $\xi_k$, $k\in\mathbb{N}$, --- независимые стандартные нормальные случайные величины, а  $\mu_k>0$ и $u_k(x)$,
$k\in\mathbb{N}$, соответственно, собственные числа и нормированные в $L_2(\mathcal{O})$ собственные функции интегрального оператора с ядром $G(s,t)$ (ковариационного оператора):
\begin{align*}
\mu_k u_k(x)=\int\limits_{\mathcal{O}}G(x,y)u_k(y)\,dy.
\end{align*}
При этом $\sum\mu_k<\infty$, т.е. ковариационный оператор принадлежит ядерному классу. Из разложения Кархунена--Лоэва немедленно следует
\begin{align}\label{S5:KL}
	\bigl\| X\bigr\|^2\stackrel{d}{=}\sum\limits_{k=1}^{\infty}\mu_k \xi_k^2.
\end{align}

Таким образом, исходная задача сводится к описанию
поведения вероятности $\mathbb{P}\{\sum_{k=1}^{\infty}\mu_k \xi_k^2\le\varepsilon^2\}$ при $\varepsilon\to 0$.
Основная трудность заключается в том, что явные формулы для собственных значений известны лишь для немногих процессов (см.~\cite{Li1992,DLL}). Если же известна достаточно точная асимптотика $\mu_k$, то асимптотика вероятности малых уклонений с точностью до константы может быть
получена с помощью принципа сравнения Венбо Ли (см.~\cite{Li1992,gao}):
\begin{prop}%{\normalfont{\cite{Li1992,gao}} }
	\label{appendix:Li}Пусть %$\xi_k$ --- последовательность независимых стандартных гауссовских с.в. , а 
	$\mu_k$ и $\tilde{\mu}_k$ --- две положительные невозрастающие суммируемые последовательности такие, что $\prod\tilde{\mu}_k/\mu_k<\infty$. Тогда
	\begin{align}\label{Li0}
	\mathbb{P}\Big\{\sum_{k=1}^{\infty} \mu_k \xi_k^2<\varepsilon^2\Big\}\sim
	\mathbb{P}\Big\{\sum_{k=1}^{\infty} \tilde{\mu}_k \xi_k^2<\varepsilon^2\Big\}
	\cdot \left( \prod\limits_{k=1}^{\infty}\frac{\tilde{\mu}_k }{\mu_k} \right)^{1/2},
	\qquad \varepsilon\to0.
	\end{align}	
\end{prop}
Мультипликативную константу из~\eqref{Li0} часто называют константой <<расхождения>> (distortion constant).
%\newpage

Следующее предложение является частным случаем ~\cite[теорема 3.1]{DLL}.
 \begin{prop}\label{thmdll}%Пусть $t,u\geq 0, d>1$ и $\delta>-1$
 	Пусть $\phi(t)$ --- определенная на $[1,\infty)$, положительная, логарифмически выпуклая, дважды дифференцируемая и интегрируемая функция. Тогда
 	\begin{align*}%\label{formulo}
 		\mathbb{P}\Big\{ \sum\limits_{k=1}^{\infty} \phi(k)\xi_k^2 \leq r  \Big\}\sim C \sqrt{\frac{f(u\phi(1))}{I_2(u)}}\exp(I_0(u)+ur),\qquad  r\to 0,
 	\end{align*}
 	где $f(t)=(1+2t)^{-1/2}$, $u=u(r)$ --- функция, удовлетворяющая соотношению
 	\begin{align} \label{u}
 		&\lim_{r\to 0}\frac{I_1(u)+ur}{\sqrt{I_2(u)}}=0,
 	\end{align}
 	а функции $I_0$, $I_1$, $I_2$ определены формулами
 	\begin{align*}
 		I_0(u)&=\int\limits_1^\infty \ln f (u \phi(t))\,dt,\\
 		I_1(u)&=\int\limits_1^\infty u \phi(t) (\ln f (u \phi(t)))'\,dt,\\
 		I_2(u)&=\int\limits_1^\infty (u \phi(t))^2 (\ln f (u \phi(t)))''\,dt.
 	\end{align*}
 \end{prop}
 Для доказательства теорем~\ref{LAP},~\ref{LOG},~\ref{NOR},~\ref{GUM},~\ref{GAM} нам потребуется частный случай предложения~\ref{thmdll}:
 \begin{prop}{\normalfont{(\cite[теорема 3.4]{Li1992}, см. также~\cite[теорема 6.2]{naznik1})}}\\
 	\label{appendix:NazNik}
 	Рассмотрим форму $\sum\limits_{n=1}^{\infty}\Lambda_k\xi_k^2$, где
 	\begin{align*}
 		\Lambda_k=(\vartheta (k+\delta))^{-d},
 	\end{align*}
 	$\vartheta>0$, $\delta>-1$, $d>1$ --- некоторые константы. Тогда при $\varepsilon\to0$
 	\begin{align*}
		\mathbb{P}\Big\{ \sum\limits_{k=0}^{\infty}\Lambda_k \xi_k^2<\varepsilon^2  \Big\}&\sim C(\vartheta,d,\delta)\cdot \varepsilon^{\gamma}\cdot \exp\Big( -\frac{d-1}{2}\Big( \frac{\pi}{d\vartheta\sin(\frac{\pi}{d})}  \Big)^{\frac{d}{d-1}}\cdot \varepsilon^{-\frac{2}{d-1}} \Big),
 	\end{align*}
 	где 
 	\begin{align*}
 	&\gamma=\frac{2-d-2d\delta}{2(d-1)},
 	&&	C(\vartheta,d,\delta)=\frac{(2\pi)^{\frac{d}{4}}\vartheta^{\frac{d\gamma}{2}}(\sin(\frac{\pi}{d}))^{\frac{1+\gamma}{2}}}{(d-1)^{\frac12}(\frac{\pi}{d})^{1+\frac{\gamma}{2}}\Gamma^{\frac{d}{2}}(1+\delta)},
 	\end{align*}
 	где $\Gamma(x)$ --- это гамма-функция.
 \end{prop}

==> S6-Bateman.tex <==
\section{Вывод формулы Бейтмана}
Пусть $\mu_k^0$ и $u_k(x)$ --- собственные числа и соответствующие им собственные функции интегрального оператора с ядром $G_{0}(x,y)$. 
Пусть ядро возмущенного оператора $G_A$ определено  по формуле \eqref{GXpert}.

\begin{thm} \textbf{(Формула Бейтмана)}
	
	Пусть $\mathcal{F}^0(z)$ и $\mathcal{F}(z)$ --- определители Фредгольма для ядер $G_0(x,y)$ и $G_A(x,y)$, соответственно. Тогда
	\begin{align}%\label{Sukhatme}
	\frac{\mathcal{F}(z)}{\mathcal{F}^0(z)}=\det (L(z)),
	\end{align}
	где матрица $L(z)$ определяется из соотношения
	\begin{align}%\label{L}
	L(z)=E_m+\sum\limits_{n=1}^{\infty}\frac{\lambda_n^0\vec{a}_n\vec{a}_n^{\,T}}{1-\frac{\lambda_n^0}{z}}\cdot D.
	\end{align}
	Здесь $E_m$ --- единичная матрица порядка $m$, а $	\vec{a}_n=\int\limits_{\mathcal{O}}\vec{\psi}(x)u_n(x)\,dx$ --- $n$-ый коэффициент Фурье вектор-функции $\vec{\psi}(x)$.
\end{thm} 
\beginproofdot
Рассмотрим $\lambda$ --- решение уравнения:
\begin{align*}
	u(x)=\lambda\int\limits_{\mathcal{O}}(G_0(x,y)+\vec{\psi}(x)^T\cdot D\cdot\vec{\psi}(y))\,u(y)\,dy
\end{align*}
Обозначим $\vec{c}(u)=\int\limits_{\mathcal{O}}\vec{\psi}(y)u(y)\,dy$, тогда имеющееся равенство можно переписать следующим образом:
\begin{align}\label{eqlambda}
u(x)=\lambda \vec{\psi}(x)^T\cdot D\cdot\vec{c}(u)+\lambda\int\limits_{\mathcal{O}}G_0(x,y)u(y)\,dy
\end{align}
Пусть $\lambda\not=\lambda_n^0$, $n\in\mathbb{N}$. Разложим все по базису $u_n(x)$. Пусть $u(x)=\sum_n\beta_n u_n(x)$. Воспользуемся представлением для ядра оператора
\begin{align*}
	G_0(x,y)=\sum\limits_{n=1}^{\infty}\frac{u_n(x)u_n(y)}{\lambda_n^0},
\end{align*}
тогда
\begin{align*}
	\sum\limits_{n=1}^{\infty}\beta_nu_n(x)=\lambda\sum\limits_{n=1}^{\infty}\vec{a}_n^{\,T}\cdot D\cdot \vec{c}(u)\;u_n(x)+\sum\limits_{n=1}^{\infty}\frac{\lambda}{\lambda_n^0}\beta_n\,u_n(x).
\end{align*}
Отсюда 
\begin{align*}
\beta_n=\frac{\lambda}{1-\frac{\lambda}{\lambda_n^0}}\cdot   \vec{a}_n^{\,T}\cdot D\cdot \vec{c}(u),\qquad u(x)=\sum\limits_{n=1}^{\infty}\frac{\lambda}{1-\frac{\lambda}{\lambda_n^0}}\cdot   \vec{a}_n^{\,T}\cdot D\cdot \vec{c}(u)\;u_n(x).
\end{align*}
Домножим последнее равенство на $\vec{\psi}(x)$ и проинтегрируем по $\mathcal{O}$, получим:
\begin{align*}
\vec{c}(u)=\sum\limits_{n=1}^{\infty}\frac{\lambda}{1-\frac{\lambda}{\lambda_n^0}}\cdot   \vec{a}_n^{\,T}\cdot D\cdot \vec{c}(u)\;\cdot\vec{a}_n,
\end{align*}
что равносильно
\begin{align*}
\vec{c}(u)+\sum\limits_{n=1}^{\infty}\frac{\lambda_n^0}{1-\frac{\lambda_n^0}{\lambda}}\cdot   \vec{a}_n^{\,T}\cdot D\cdot \vec{c}(u)\;\cdot\vec{a}_n=0.
\end{align*}
Запишем покоординатно ($k=1,\ldots,m$):
\begin{align*}
c_k(u)+\sum\limits_{n=1}^{\infty}\frac{\lambda_n^0}{1-\frac{\lambda_n^0}{\lambda}}\cdot   \vec{a}_n^{\,T}\cdot D\cdot \vec{c}(u)\;\cdot (a_k)_n=0,
\\
c_k(u)+\sum\limits_{n=1}^{\infty}\frac{\lambda_n^0}{1-\frac{\lambda_n^0}{\lambda}}\sum\limits_{i,j=1}^m   (a_i)_n\cdot D_{ij}\cdot c_j(u)\;\cdot (a_k)_n=0,
\\
c_k(u)+\sum\limits_{j=1}^m c_j(u)\sum\limits_{n=1}^{\infty}\frac{\lambda_n^0}{1-\frac{\lambda_n^0}{\lambda}}\sum\limits_{i=1}^m   (a_i)_n\cdot D_{ij}\cdot  (a_k)_n =0,
\end{align*}
что равносильно тому, что $L(\lambda)\cdot\vec{c}(u)=0$.  Если $\vec{c}(u)=0$, то из \eqref{eqlambda} следует, что $\lambda=\lambda_n^0$ (а мы предположили противное). Тогда у системы существует нетривиальное решение и должно выполняться $\det(L)=0$.
\begin{rem}
	Пока мы доказали, что все корни целой функции $\mathcal{F}(z)$ являются корнями функции $\mathcal{F}^0(z)\cdot\det(L(z))$. Нужно еще доказать в обратную сторону. Мы этого сейчас делать не будем, т.к. нам необходим только сам вид функции $L(z)$. Подробнее о том, как это делать, можно найти, например, в \cite{darling1955}.
\end{rem}
\endproof

